Selective excitation of high-order modes in two-dimensional cavity resonator integrated grating filters

The selective spatial mode excitation of a bi-dimensional grating-coupled micro-cavity called a Cavity Resonator Integrated Grating Filter (CRIGF) is reported using an incident beam shaped to reproduce the theoretical emission profiles of the device in one- and subsequently two-dimensions.In both cases, the selective excitation of modes up to order 10 (per direction) is confirmed by responses exhibiting one (respectively two) spectrally narrow-band resonance(s) with a good extinction of the other modes, the latter being shown to depend on the parity and order(s) of the involved modes. These results paves the way towards the demonstration of multi-wavelength spatially-selective reflectors or fibre-to-waveguide couplers. Also, subject to an appropriate choice of the materials constituting the CRIGF, this work can be extended to obtain mode-selectable laser emission or nonlinear frequency conversion.

==> MANIFEST <==
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\biblio.bib
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\CRIGF_img.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\gaussian_scanning_map.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\matrix_cross_correl.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\polar_45deg.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\spectra.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\images\spectra_2D.pdf
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\main.bbl
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\main.bib
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\main.out
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\main.tex
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\main.xwm
C:\Users\antoi\Documents\travail\arxiv_submissions\crigf_OL\preprint.sty

